On the Need for Topology-Aware Generative Models for Manifold-Based Defenses

Machine-learning (ML) algorithms or models, especially deep neural networks (DNNs), have shown significant promise in several areas. However, researchers have recently demonstrated that ML algorithms, especially DNNs, are vulnerable to adversarial examples (slightly perturbed samples that cause misclassification). The existence of adversarial examples has hindered the deployment of ML algorithms in safety-critical sectors, such as security. Several defenses for adversarial examples exist in the literature. One of the important classes of defenses are manifold-based defenses, where a sample is ``pulled back" into the data manifold before classifying. These defenses rely on the assumption that data lie in a manifold of a lower dimension than the input space. These defenses use a generative model to approximate the input distribution. In this paper, we investigate the following question: do the generative models used in manifold-based defenses need to be topology-aware? We suggest the answer is yes, and we provide theoretical and empirical evidence to support our claim.

==> section/background/background-den.tex <==
\vspace{-5pt}
\subsection{Density from a data-generating manifold}
\vspace{-5pt}
\label{sec-prob-manifold}

%\paragraph{Probability over a Riemannian manifold.}
    We first compute a probability of $\bfx$ being generated from a Riemannian manifold $M$, without noise.
    We assume a $k$-dimensional manifold $M$ equipped with a Riemannian metric $g$, a family of inner products $g_{\bfx}$ on tangent spaces $T_{\bfx}M$.
    In this case, $g$ induces the volume measure $dM$ for integration over $M$.
    If $M$ is parameterized by $\bfx=X(\bfu)$ for $\bfu\in D\subseteq\bbR^k$, the integration of a density function $p$ on $M$ is as follows.
    {\small
    \begin{align}
        \label{eq-int-volume-form}
        \int_{\bfx\in M}p(\bfx)dM(\bfx)=\int_{\bfu\in D}p(X(\bfu))\sqrt{\left|\det[g_{X(\bfu)}]\right|}d\bfu
    \end{align}
    }
    where $[g_{X(\bfu)}]$ is the $k\times k$ matrix representation of the inner product $g_{X(\bfu)}$ at $X(\bfu)\in M$.

    In section \ref{sec-example}, a concrete example of this computation will be provided.

\iffalse
\paragraph{Computing density $p$ over a Riemannian manifold $M$.}
    \label{sec-ex-man-density}

    This section presents example computations of the probability computations from the Section \ref{sec-prob-manifold} and \ref{sec-prob-extension}
    As a concrete example of computing density over a manifold, we use the following simple manifolds, so called \emph{two-moons} in $\bbR^2$.
    {\scriptsize
    \begin{align*}
        M_0 &= \left\{(x_1, x_2)\middle\vert \begin{array}{l}x_1=\cos\theta \\ x_2=\sin\theta\end{array}\text{ for }\theta\in[0,\pi]\right\}\\
        M_1 &= \left\{(x_1, x_2)\middle\vert \begin{array}{l}x_1=1-\cos\theta \\ x_2=1-\sin\theta+\frac{1}{2}\end{array}\text{ for }\theta\in[0,\pi]\right\}
    \end{align*}
    }
    We take $M=M_0\cup M_1$ as our example manifold.
    Figure \ref{fig-manifold} shows the manifold of two-moons dataset plotted in different colors: $M_0$ in red and $M_1$ in blue.
    \begin{figure}[hbt!]
        \centering
        \begin{subfigure}[b]{0.3\linewidth}
            \includegraphics[width=\linewidth]{image/manifold.jpg}
            \caption{Plot of the two-moons manifold in $\bbR^2$}
            \label{fig-manifold}
        \end{subfigure}
        \hspace{1em}
        \begin{subfigure}[b]{0.4\linewidth}
            \includegraphics[width=\linewidth]{image/density.jpg}
            \caption{Extended density function over $\bbR^2$ from the two-moons dataset}
            \label{fig-density}
        \end{subfigure}
        \caption{Density extension example from two-moons manifold.}
    \end{figure}

    First recall the following equation (equation (\ref{eq-int-volume-form}) from the Section \ref{sec-prob-manifold}).
    {\small
    \begin{align*}
        \int_{\bfx\in M}p(\bfx)dM(\bfx)=\int_{\bfu\in D}p(X(\bfu))\sqrt{\left|\det[g_{X(\bfu)}]\right|}d\bfu
    \end{align*}
    }
    where $[g_{X(\bfu)}]$ is the $k\times k$ matrix representation of the inner product $g_{X(\bfu)}$ at $X(\bfu)\in M$.

    Especially, when a manifold in $\bbR^n$ is of dimension 1, i.e. parameterized curve $\gamma:[a,b]\rightarrow \bbR^n$, the integration (\ref{eq-int-volume-form}) can be written in simpler way.
    {\small
    \begin{align}
        \label{eq-int-curve}
        \int_{\bfx\in M}p(\bfx)dM(\bfx)=\int_{t=a}^b p(\gamma(t))\|\gamma'(t)\|dt
    \end{align}
    }
    where $\gamma'(t)$ is the $n$-dimensional velocity vector at $t\in[a,b]$.

    Let $p$ be a probability density function defined on $M$.
    As $M$ is composed of two disjoint manifolds $M_0$ and $M_1$, we consider conditional densities $p_0, p_1$ as follows.
    {\small
    \begin{align}
        \label{eq-cond-density}
        \begin{split}
        p_0(\bfx)&=p(\bfx\vert\bfx\in M_0)=\frac{p\vert_{M_0}(\bfx)}{\Pr[\bfx\in M_0]}\\
        p_1(\bfx)&=p(\bfx\vert\bfx\in M_1)=\frac{p\vert_{M_1}(\bfx)}{\Pr[\bfx\in M_1]}
        \end{split}
    \end{align}
    }
    Here, $p\vert_{M_0}$ and $p\vert_{M_1}$ are the density function $p$ with its domain restricted to $M_0$ and $M_1$, respectively.
    By our definition of data-generating manifolds, $\Pr[\bfx\in M_i]$ corresponds to the probability of data generation for class $i$, i.e. $\Pr[y=i]$.
    For a concrete example of such density, uniform density for each manifold $M_i$ can be defined as $p_i(\bfx)=\frac{1}{\pi}$ for all $\bfx\in M_i$.

    Note that each of manifolds are parameterized curves in $\bbR^2$,
    {\small
    \begin{align*}
        \gamma_0:\theta&\mapsto(\cos\theta,\sin\theta)\\
        \gamma_1:\theta&\mapsto(1-\cos\theta,1-\sin\theta+0.5)
    \end{align*}
    }
    with constant speed $\|\gamma_0'(\theta)\|=\|\gamma_1'(\theta)\|=1$ at all $\theta\in [0,\pi]$.
    Therefore, from equation (\ref{eq-int-curve}),
    {\small
    \begin{align}
        \label{eq-int-example}
        \begin{split}
            \int_{\bfx\in M_0}p\vert_{M_0}(\bfx)dM_0(\bfx)=\int_{\theta=0}^\pi p(\gamma_0(\theta))d\theta\\
            \int_{\bfx\in M_0}p\vert_{M_1}(\bfx)dM_1(\bfx)=\int_{\theta=0}^\pi p(\gamma_1(\theta))d\theta
        \end{split}
    \end{align}
    }

    For any measurable subset $A\subseteq M$, the probability for an event that $\bfx$ is in $A$ can be computed as follows.
    {\small
    \begin{align*}
        \Pr[\bfx\in A]=&\int_{\bfx\in A\subseteq M}p(\bfx)dM(\bfx)\\
        =&\int_{\bfx\in A\cap M_0}p\vert_{M_0}(\bfx)dM_0(\bfx)+\int_{\bfx\in A\cap M_1}p\vert_{M_1}(\bfx)dM_1(\bfx)\\
        =&\int_{\substack{\theta\in [0,\pi]\\\gamma_0(\theta)\in A}}p\vert_{M_0}(\gamma_0(\theta))d\theta+\int_{\substack{\theta\in [0,\pi]\\\gamma_1(\theta)\in A}}p\vert_{M_1}(\gamma_1(\theta))d\theta\quad(\because\text{(\ref{eq-int-example})})\\
        =&\Pr[\bfx\in M_0]\int_{\substack{\theta\in [0,\pi]\\\gamma_0(\theta)\in A}}p_0(\gamma_0(\theta))d\theta\\
        &+\Pr[\bfx\in M_1]\int_{\substack{\theta\in [0,\pi]\\\gamma_1(\theta)\in A}}p_1(\gamma_1(\theta))d\theta\quad(\because\text{(\ref{eq-cond-density})})\\
        =&\frac{1}{\pi}\left(\Pr[\bfx\in M_0]\int_{\substack{\theta\in [0,\pi]\\\gamma_0(\theta)\in A}}1 d\theta
        +\Pr[\bfx\in M_1]\int_{\substack{\theta\in [0,\pi]\\\gamma_1(\theta)\in A}}1 d\theta\right)
    \end{align*}
    }
    We can briefly check all the requirements \ref{req-man-1}, \ref{req-man-2}, and \ref{req-man-3}.
    The computation of $\Pr[\bfx\in A]$ is based on \ref{req-man-1}, so \ref{req-man-1} is satisfied trivially.
    Also, $p$ is a function defined only on $M$, thus \ref{req-man-2} is clear, i.e. ${\rm supp}(p) = \{\bfx\in\bbR^n\mid p(\bfx)>0\} \subseteq M$.
    To check \ref{req-man-3}, when $A=M_i$, computing this integration will result in the exact probability $\Pr[\bfx\in M_i]=\Pr[y=i]$, so when $A=M$, computing the integration will result in $\Pr[y=0]+\Pr[y=1]=1$, as desired in the requirements.
\fi


==> section/background/background-dis.tex <==
\vspace{-5pt}
\subsection{Discussion on the extended density}
\vspace{-5pt}
    This section introduces some remaining discussions regarding our data-generating process from a data-generating manifold.
    \paragraph{Relation to kernel density estimation.}
        While this extension is computing the density of compound distribution, it can be interpreted as computing expectation over a family of locally defined densities.
        Such expected value can be observed in previous approaches of density estimation.
        For example, if $\nu_{\bfx}$ is isotropic Gaussian for each $\bfx$, the above integration is equivalent to the kernel density estimation, with Gaussian kernel, over infinitely many points on $M$.
        We may also consider a set of multivariate Gaussian noises that are locally flattened to reflect the tangent space of manifold, the above integration is equivalent to density estimation using manifold Parzen window~\citep{vincent2003manifold}.

    \paragraph{Observed property of the extended density.}
        In Figure \ref{fig-density} in Section \ref{sec-ex-man-density}, we can observe that the extended density achieved higher values near the data-generating manifold.
        We formalize this observation to discuss its implication to the INC approach.

        Let $d(\hat\bfx,M)$ to be the minimum distance from $\hat\bfx$ to the manifold $M$.
        \begin{enumerate}[start=1, label={(\bfseries C\arabic*)}]
            \item \label{cond-prop-1}
            For any given $\hat\bfx$, let $y^*$ be the class label whose conditional density $p_M(\hat\bfx|y=y*)$ dominates $p_M(\hat\bfx|y=i)$ for $i\not=y^*$,
            {\small
            \begin{align}
                y^*\in\arg\max_{i\in[l]}p_M(\hat\bfx|y=i)
            \end{align}
            }
            and let $M_{y^*}$ be the manifold corresponding to $y^*$.
            \item \label{cond-prop-2}
            For $y^*$ satisfying \ref{cond-prop-1}, we choose $y^*$ such that the distance of $\hat\bfx$ from the manifold $d(\hat\bfx, M_{y^*})$ is the smallest.

        \end{enumerate}
        If there are multiple $y^*$ satisfying both of \ref{cond-prop-1} and \ref{cond-prop-2}, we expect the following property to be true for all of those $y^*$.
        \begin{enumerate}[start=1, label={(\bfseries P\arabic*)}]
            \item \label{prop-discussion}
            Consider the shortest line from $\hat\bfx$ to the manifold $M_{y^*}$.
            As $\hat\bfx$ goes closer to $M_{y*}$ along this line, $\hat\bfx$ should be more likely to be generated as the influence of noise decreases when moving away from the manifold.
            Therefore, we expect our density $p_M$ to have the following property.
            {\small
            \begin{align}
                \label{prop-implication}
                \begin{split}
                &\bfx^*\in\arg\min_{\bfx\in M_{y^*}}d(\hat\bfx,\bfx)\\
                \implies&p_M(\hat\bfx)\le p_M((1-\lambda)\hat\bfx + \lambda\bfx^*)\text{ for all }\lambda\in[0,1]
                \end{split}
            \end{align}
            }
        \end{enumerate}
        Actually, this provides another justification of INC.
        In reality, the density conditioned by the label is not available even after running a generative model, so finding $y^*$ with \ref{cond-prop-1} is relatively hard.
        If we only consider \ref{cond-prop-2} without filtering $y^*$ via \ref{cond-prop-1}, we are finding a point $\bfx\in M$ achieving the minimum distance to $\hat\bfx$, which is the optimization (\ref{inc-ideal}) above.
        Then projecting $\hat\bfx$ to the $\bfx^*$, i.e. the solution of the optimization \ref{inc-ideal}, can be explained by \ref{prop-implication}; when $\lambda=1$, $p_M$ is the highest along the shortest line between $\hat\bfx$ and $\bfx^*$.

==> section/expr-mnist.tex <==
    We demonstrate the effectiveness of INC with class-aware generative models, especially when applied to data of higher dimension.
    Specifically, we first train a classifier on MNIST dataset consisting of $28\times 28$ grayscale images of handwritten digits.
    Then, we measure the INC defense rate against known attacks, e.g. FGSM.

    We trained an MNIST model using the example code in {\sf Keras}, then we generated adversarial examples using attack algorithms implemented in the {\sf Foolbox} package.
    For the attack method, we used FGSM and PGD, performing line search of step size 0.0003 from 0 to the maximum perturbation size 0.3 in $\ell^\infty$-norm.
    (Each data point was normalized to have $[0,1]$ range)
    When evaluated over MNIST testset containing 10000 images, the trained model has 99.130 \% accuracy before the attack, and the accuracy drops to 0.009 \% after applying FGSM attack.
    
    To train generative models, we implemented two RealNVP models of four coupling layers using {\sf Tensorflow Probability} library.
    Each coupling layer contains 8 hidden layers of 1024 units.
    We also permuted dimensions before passing data into each coupling layers, to implement checkerboard masking of RealNVP.
    Each model was trained with 16000 iterations with learning rate $5\times 10^{-7}$, randomly sampling training batch of 1000 different data points for each iteration.
    
    To test the defense rate, we sampled 1000 point that the attack was successful, then run 100 iterations of INC optimization for each of adversarial points.
    
    \textcolor{red}{(Add experimental results after projection is finished.)}


==> section/unused/theory-gen.tex <==
\subsection{Generalization of the Theorem \ref{thm-diff}}
    The Theorem \ref{thm-diff} mainly uses a fact that the number of connected components of $\lambda$-density level set is preserved by a continuous generative model $G$.

    In algebraic topology, each connected component corresponds to a generator of $0$-th homology group $H_0$, and continuity of a function is enough to preserve each component.
    In general, generators of $i$-th homology group $H_i$ for $i>0$ are not preserved by a continuous map, so we need to restrict $G$ further.
    By requiring $G$ to be a homeomorphism, we can safely guarantee that all topological properties are preserved by $G$, therefore we can generalize the Theorem \ref{thm-diff} with a homeomorphic generative model $G$.

    To generalize the proof of the Theorem \ref{thm-diff}, we first provide the sketch of the proof.
    \vspace{-5pt}
    \begin{enumerate}[label={\bfseries (\arabic*)}]
        \setlength\itemsep{0em}
        \item \label{step-1} $\lambda^*$-density level set $L_{\lambda^*}^Z$ of mixture of Gaussian has at most $n_Z$ connected component.
        \item \label{step-2} Since $G$ is continuous, the number of connected components of $L_{\lambda^*}^G(Z)=G(L_{\lambda^*}^Z)$ is same to the number of connected components of $L_{\lambda^*}^Z$, so it is also at most $n_Z$.
        \item \label{step-3} We chose $\lambda^*$ so that $L_{\lambda^*}^X$ is included in $\delta^*$-neighborhood of $M$.
        \item \label{step-4} By assumption on the class-wise distance of $M$, $\delta^*$-neighborhood of $M$ has exactly same number of connected components to $M$, i.e. $n_X$. Therefore $L_{\lambda^*}^X$ has at least $n_X$ connected components.
        \item \label{step-5} By \ref{step-2} and \ref{step-4}, we conclude that $L_{\lambda^*}^G(Z)$ and $L_{\lambda^*}^X$ do not agree on the number of connected components as long as $n_Z < n_X$.
    \end{enumerate}
    \vspace{-5pt}
    In this proof, $n_Z$ corresponds to the maximal $0$-th Betti number of $L_{\lambda^*}^Z$, i.e. the number of generators of $H_0(L_{\lambda^*}^Z)$.
    If we keep using a mixture of Gaussians as latent vector distribution, all components of $L_{\lambda^*}^Z$ are contractible, so we may use $0$ as the maximal $i$-th Betti number.

    Also, $n_X$ corresponds to the $0$-th Betti number of $M$ and it worked as the minimal $0$-th Betti number of $L_{\lambda^*}^X$.
    The condition on the class-wise distance of $M$ is used to ensure $n_X$ to be a lower bound.
    Combining these observations, we can get the following generalized statement.
    \begin{theorem}
        \label{thm-generalized}
        Let $\calD_Z$ be a mixture of multivariate Gaussian distributions, and let $\calD_X$ be the target distribution from data-generating manifold $M$.
        Let $n_i$ be the $i$-th Betti number of $M$.

        Consider a generative model $G$ is used to approximate $\calD_X$ using the latent vectors sampled from $\calD_Z$.
        Assume that $G$ is a homeomorphism from $\bbR^n$ to itself.
        Assume that data-generating manifold satisfies the conditions of the Theorem \ref{thm-man-separation}, and let $\lambda^*$ be the threshold value that $L_{\lambda^*}^X$ corresponds to that level set.
        Assume that for some $j>0$, the homomorphism $\iota^*$ induced by the inclusion $\iota:M\rightarrow N_{\delta^*}(M)$ is injective.
        \footnote{Any generator of the $j$-th homology group $H_j(M)$ of $M$ is mapped to a nonzero generators of the $j$-th homology group $H_j(N_{\delta^*}(M))$ of $\delta^*$-neighborhood of $M$.}

        If $0<n_j$, $L_{\lambda^*}^X$ and $L_{\lambda^*}^{G(Z)}$ do not agree on the number of connected component.
    \end{theorem}
    \begin{proof}
        Since $L_{\lambda^*}^X$ is the results of Theorem \ref{thm-man-separation}, it includes $M$ and is included by $\delta^*$-neighborhood $N_{\delta^*}(M)$ of $M$.
        %Since $L_{\lambda^*}^X$ includes $M$, all generator of $j$-th homology group of $M$ is at least contained in $M$.
        Define inclusions $\iota_1, \iota_2$ as,
        \vspace{-5pt}
        \begin{itemize}
            \setlength\itemsep{0em}
            \item $\iota_1:M\rightarrow L_{\lambda^*}^X$
            \item $\iota_2:L_{\lambda^*}^X\rightarrow N_{\delta^*}(M)$
        \end{itemize}
        \vspace{-5pt}
        Clearly, $\iota = \iota_2\circ\iota_1$.

        Let $\iota_1^*$ and $\iota_2^*$ be induced homomorphisms of $\iota_1$ and $\iota_2$, resp.

        By the assumption, any generator $[a]$ in $H_j(M)$ is injectively mapped to a nonzero generator $\iota^*([a])$ in $H_j(N_{\delta^*}(M))$.
        Therefore, the $j$-th Betti number of $N_{\delta^*}(M)$ is equal to that of $M$, i.e. $n_j$.
        Note that $j$-th Betti number is the rank of $j$-th homology group $\text{rank}(H_j(N_{\delta^*}(M)))$
        Because $\iota_2^*$ is a homomorphism from $H_j(L_{\lambda^*}^X)$ to $H_j(N_{\delta^*}(M))$, $\text{rank}(L_{\lambda^*}^X)\ge\text{rank}(H_j(N_{\delta^*}(M)))$.
        Therefore the $j$-th Betti number of $L_{\lambda^*}^X$ is at least $n_j$.

        However, since $\calD_Z$ is a mixture of Gaussians, for any value of $\lambda$ (including the special case $\lambda=\lambda^*$), $L_{\lambda}^Z$ does not have any generator of $j$-th homology group, so it has $j$-th Betti number $0$ for all $j>0$.
        Since $G$ is homeomorphic, it preserves all the Betti numbers, thus $L_{\lambda^*}^{G(Z)}=G(L_{\lambda^*}^Z)$ has the same $j$-th Betti number.
        As $0<n_j$, $L_{\lambda^*}^X$ and $L_{\lambda^*}^{G(Z)}$ can never agree on the number of connected components.
    \end{proof}
    Later in Section \ref{sec-expr-1}, we will see the Figure \ref{fig-level-set-circles-ca} from the circles dataset, which is a remarkable example that $L_{\lambda}^G(Z)$ has the same number of connected components, but does not have any loop (non-contractible circle).
    This is empirical evidence of the Theorem \ref{thm-generalized}, so it is explained by mismatches in the topology of distributions.
    Each concentric circle has $\mathbb{Z}$ as its first homology group as circle contains exactly one generator.
    However, latent vector distribution always has a trivial first homology group, as any level set of a mixture of Gaussians is a set of contractible connected components.

